New bounds for range closest-pair problems

Given a dataset $S$ of points in $\mathbb{R}^2$, the range closest-pair (RCP) problem aims to preprocess $S$ into a data structure such that when a query range $X$ is specified, the closest-pair in $S \cap X$ can be reported efficiently. The RCP problem can be viewed as a range-search version of the classical closest-pair problem, and finds applications in many areas. Due to its non-decomposability, the RCP problem is much more challenging than many traditional range-search problems. This paper revisits the RCP problem, and proposes new data structures for various query types including quadrants, strips, rectangles, and halfplanes. Both worst-case and average-case analyses (in the sense that the data points are drawn uniformly and independently from the unit square) are applied to these new data structures, which result in new bounds for the RCP problem. Some of the new bounds significantly improve the previous results, while the others are entirely new.

==> figure_page.tex <==
\newpage
{\noindent \bf \LARGE \textsc{Figure Pages}}

\begin{figure}[h]
	\begin{center}
		\subfloat[Corners of weighted quadrants $\{W_1, \dots, W_6\}$, indexed by increasing weight.]{
			\includegraphics[height=4cm]{2_sided_init.eps}
			\label{figure:2-sided init}
		}
		\hspace{1cm}
		\subfloat[The subdivision $\mathcal{A}$ induced by quadrants $\{W_1, \dots, W_6\}$.]{
			\includegraphics[height=4cm]{2_sided_subdivision.eps}
			\label{figure:2-sided subdivision}
		}
	\end{center}
	\caption{Illustrating weighted quadrants and their induced subdivision.}
	\label{figure:weighted quadrant}
\end{figure}

% \begin{figure}[h]
% 	\begin{center}
% 		\subfloat[Case 1]{
% 			\includegraphics[height=2cm]{3_sided_linear_1.eps}
% 		}
% 		\hspace{0.5cm}
% 		\subfloat[Case 2]{
% 			\includegraphics[height=2cm]{3_sided_linear_2.eps}
% 		}
% 		\hspace{0.5cm}
% 		\subfloat[Case 3]{
% 			\includegraphics[height=2cm]{3_sided_linear_3.eps}
% 		}
% 	\end{center}
% 	\caption{Illustrating the three cases of Lemma~\ref{lemma:n pairs if flat}
% 	}
% 	\label{figure:n pairs if flat}
% \end{figure}



\begin{figure}[H]
	\begin{center}
		\subfloat[Pair $(a_i, b_i)$ is in halfplane $Q$ iff $l^*$ is in the upward-open wedge $W_i$ formed by $a_i^*$ and $b_i^*$.]{
			\includegraphics[]{halfspace_open_wedge.eps}
			\label{figure:halfspace open wedge}
		}
		\hspace{0.5cm}
		\subfloat[As illustration of Case (1)]{
			\includegraphics[]{halfspace_case_1.eps}
			\label{figure:halfspace case 1}
		}
						\hspace{0.5cm}
		\subfloat[Moving $p$ and rotating line $a_ib_i$ clockwise around $a_i$]{
			\includegraphics[]{halfspace_case_2_1.eps}
			\label{figure:halfspace case 2 1}
		}
		\hspace{0.5cm}
		\subfloat[An example for Case (2) where $r \cap W_j = \emptyset$.]{
			\includegraphics[]{halfspace_case_2_2.eps}
			\label{figure:halfspace case 2 2}
		}  

	\caption{Illustrating the various cases in Theorem~\ref{theorem:wedge arrangement is planar}.}
	
	\end{center}
\end{figure}

\begin{figure}[H]
	\ContinuedFloat
\begin{center}

		\hspace{0.5cm}
		\subfloat[An example for Case (2) where $r \cap W_j \neq \emptyset$.]{
			\includegraphics[]{halfspace_case_2_3.eps}
			\label{figure:halfspace case 2 3}
		}  
		\hspace{0.5cm}
		\subfloat[An example for Case (3) where $a_jb_j$ is to the left and $r \cap W_j = \emptyset$.]{
			\includegraphics[]{halfspace_case_3_1.eps}
			\label{figure:halfspace case 3 ajbj intersects aibi and to the left}
		} 
		\hspace{0.5cm}
		\subfloat[An example for Case (3) where $(l_i')^* \not\in r$ and $r \cap W_j = \emptyset$.]{
			\includegraphics[]{halfspace_case_3_2.eps}
			\label{figure:halfspace case 3, l does not exist in r}
		}     
		\hspace{0.5cm}
		\subfloat[An example for Case (3) where $(l_i')^* \not\in r$ and $r \cap W_j \neq \emptyset$.]{
			\includegraphics[]{halfspace_case_3_3.eps}
			\label{figure:halfspace case 3, l does not exist in r, another}
		}
		\hspace{0.5cm}
		\subfloat[An example for Case (3) where $(l_i')^* \in r$ and $r \cap W_j$ contains $(l_i')^*$ but does not contain $r_0$ or the infinite end of $r$.]{
			\includegraphics[]{halfspace_case_3_4.eps}
			\label{figure:halfspace case 3, l in r}
		}                
	\end{center}
	\caption{Illustrating the various cases in Theorem~\ref{theorem:wedge arrangement is planar} (continued).}
\end{figure}



\begin{figure}[h]
	\setcounter{subfigure}{0}
	\centering
	\subfloat[Plainly intersect] {
		\includegraphics[height=2.3cm]{plain_1.pdf}
	}
% 	\subfloat[Plainly intersect] {
% 	\includegraphics[height=2cm]{plain_2.pdf}
% }
    \hspace{1cm}
	\subfloat[Not plainly intersect] {
	\includegraphics[height=2.3cm]{plain_3.pdf}
}
% 	\subfloat[Not plainly interesect] {
% 	\includegraphics[height=2cm]{plain_4.pdf}
% }
\caption{An illustration of ``plainly intersect''}
\label{figure:plainly intersect}
\end{figure}

% TODO
% Yuan
\begin{figure}[H]
	\setcounter{subfigure}{0}
	\centering
	\subfloat[A line with a strictly $C$-vanishing side and a side that is not $C$-vanishing] {
		\includegraphics[height=3.7cm]{vanish_1.pdf}
	}
    \hspace{2cm}
	\subfloat[A line with two $C$-vanishing sides] {
	\includegraphics[height=3.7cm]{vanish_2.pdf}
}
\caption{An illustration of ``$C$-vanishing''}
\label{figure:vanishing}
\end{figure}

\newpage
